Exploring External Knowledge for Accurate modeling of Visual and Language Problems

The interest in Artificial Intelligence (AI) and its applications has seen unprecedented growth in the last few years. The success can be partly attributed to the advancements of deep neural networks made in the sub-fields of AI such as Computer Vision (CV) and Natural Language Processing (NLP). The promising research area that this dissertation focuses on is visual and language understanding which involves many challenging tasks, i.e., classification, detection, segmentation, machine translation and captioning, etc. The state-of-the-art methods for solving these problems usually involves only two parts: source data and target labels, which is rather insufficient especially when the dataset is small. Meanwhile, many external tools or sources can provide extra useful information (external knowledge) that can help improve the performance of these methods. For example, a detection model has been applied to provide better object features than state-of-the-art ResNet for image captioning models. Inspired by this observation, we developed a methodology that we can first extract external knowledge and then integrate it with the original models. The external knowledge has to be extracted from the dataset, or can directly come from external, e.g., grammar rules or scene graphs. We apply this methodology to different AI tasks, including machine translation and image captioning and improve the original state-of-the-art models by a large margin.

==> Chapter1/chapter1.tex <==
% \newpage








==> Chapter3/abstract.tex <==

State-of-the-art techniques in Generative Adversarial Networks (GANs) have shown remarkable success in image-to-image translation from peer domain \textit{X} to domain \textit{Y} using paired image data. However, obtaining abundant paired data is a non-trivial and expensive process in the majority of applications. When there is a need to translate images across $n$ domains, if the training is performed between every two domains, the complexity of the training will increase quadratically. Moreover, training  with data from two domains only at a time cannot benefit from data of other domains, which prevents the extraction of more useful features and hinders the progress of this research area. In this work, we propose a general framework for unsupervised image-to-image translation across multiple domains, which can translate images from domain $X$ to any a domain without requiring direct training between the two domains involved in image translation. A byproduct of the framework is the reduction of computing time and computing resources, since it needs less time than training the domains in pairs as is done in state-of-the-art works. Our proposed framework consists of a pair of encoders along with a pair of GANs which learns high-level features across different domains to generate diverse and realistic samples from. Our framework shows competing results on many image-to-image tasks compared with state-of-the-art techniques. 



==> Chapter4/abstract.tex <==

Learning target side syntactic structure has been shown to improve Neural Machine Translation (NMT). However, incorporating syntax through latent variables introduces additional complexity in inference, as the models need to marginalize over the latent syntactic structures. To avoid this, models often resort to greedy search which only allows them to explore a limited portion of the latent space.

In this work, we introduce a new latent variable model, \name, that captures the co-dependence between syntax and semantics, while allowing for effective and efficient inference over the latent space. \name decouples direct dependence between successive latent variables, which allows its decoder to exhaustively search through the latent syntactic choices, while keeping decoding speed proportional to the size of the latent variable vocabulary.
We implement \name by modifying a transformer-based NMT system and design a neural expectation maximization algorithm that we regularize with part-of-speech information as the latent sequences. 
Evaluations on four different MT tasks show that incorporating target side syntax with \name improves both translation quality, and also provides an opportunity to improve diversity. 



















==> Chapter5/1_abstract.tex <==
Generating accurate descriptions for online fashion items is important not only for enhancing customers' shopping experiences, but also for the increase of online sales. 
Besides the need of correctly presenting the attributes of items, the expressions in an enchanting style could better attract customer interests.
The goal of this work is to develop a novel learning framework for accurate and expressive fashion captioning. 
Different from popular work on image captioning, it is hard to identify and describe the rich attributes of fashion items.
We seed the description of an item by first identifying its attributes, and introduce
\textit{attribute-level semantic} (ALS) reward and \textit{sentence-level semantic} (SLS) reward as metrics to improve the quality of text descriptions. 
We further integrate the training of our model with maximum likelihood estimation (MLE), attribute embedding, and Reinforcement Learning (RL).
To facilitate the learning,  we build a new FAshion CAptioning Dataset (FACAD), which contains $800$K images and $120$K corresponding enchanting and diverse descriptions.
Experiments on FACAD demonstrate the effectiveness of our model.

==> Chapter6/60_abstract.tex <==

The task of news article image captioning aims to generate descriptive and informative captions for news article \textit{images}. 
Unlike conventional image captions that simply describe the content of the image in general terms, news image captions follow journalistic guidelines and rely heavily on named entities to describe the image content, often drawing context from the whole article they are associated with. 
%Thus, the specific structure and content of news image captions makes this task particularly challenging.
%news article image captioning especially challenging.
%Thus, the specific structure and content of news image captions make news article image captioning especially challenging.
In this work, we propose a new approach to this task, motivated by caption guidelines that journalists follow.
Our approach, \fullname (\name), leverages the %underlying journalistic 
structure of captions to improve the generation quality and guide our representation design.
%explain the corresponding process.
% template-driven caption generation, named entities and contextual information contained throughout the news article.
%In this work, we propose \fullname (\name) that  integrates the editorial guidelines  with a templated caption generation process, and
% structure of captions with the most common `template' components 
% (\textit{who}, \textit{when}, \textit{where}, \textit{context}, and \textit{miscellaneous}) 
%exploits both named entities and contextual information contained throughout the news article 
 %illustrated by the image
 %in the encoding step of our approach.
Experimental results, including detailed ablation studies, on two large-scale publicly available datasets show that \name substantially outperforms state-of-the-art methods both on
caption generation and named entity related metrics.


==> Chapter7/1_abstract.tex <==

Image captioning is shown to be able to achieve a better performance by using scene graphs to represent the relations of objects in the image.
%Exploring object relationships for captioning images has achieved some progress by using scene graphs as the external knowledge and has yielded better performances than non-relational image captioners.
% However, to make full use of the scene graphs and design a more powerful model especially a better encoder is still under-explored.
% However, how to design a model that can better integrate the scene graphs is still under-explored.
The current captioning encoders generally use a Graph Convolutional Net (GCN) to represent the relation information and merge it with the object region features via concatenation or convolution to get the final input for sentence decoding.
% However, it is more appropriate to train the GCN with a relational objective to get better relation features rather than only with one image captioning objective.
However, the GCN-based encoders in the existing methods are less effective for captioning due to two reasons. First, using the image captioning as the objective (i.e., Maximum Likelihood Estimation) rather than a relation-centric loss cannot fully explore the potential of the encoder. Second, using a pre-trained model instead of the encoder itself to extract the relationships is not flexible and cannot contribute to the explainability of the model.
% \rev{However, the image captioning objective (i.e., Maximum Likelihood Estimation) itself cannot fully
% explore the potential of the encoders since it is not a relationcentric metric. Meanwhile, they ignore the importance of
% using the encoder to explicitly express the pair-wise relationships, which can make the whole captioner more explainable.}
%Meanwhile, they ignore the importance of using the encoder to explicitly express the pair-wise relationships, which can make the whole captioner more explainable. 
% Meanwhile, they ignore the importance of using the encoder to explicitly express the pair-wise relationships, which can help the decoder to better understand how to use a specific relational word.
% Meanwhile, concatenating the relation information encoded via GCN with the object features make the relation expression less obvious since only with the final image feature we cannot tell the pair-wise relationships any more. 
To improve the quality of image captioning, we propose a novel architecture \name - a RElational transFORMER to generate features with relation information embedded and to explicitly express the pair-wise relationships between objects in the image.
\name incorporates the objective of scene graph generation with that of image captioning using one modified Transformer model.
% whose encoder is first pre-trained during the scene graph generation phase and then the whole model is continuously trained using the image captioning loss with an auxiliary scene graph generation objective.
This design allows \name to generate not only better image captions with the benefit of extracting strong relational image features, but also scene graphs to explicitly describe the pair-wise relationships.
% Our model is the first work to use a Transformer to generate image captions as well as scene graphs.
Experiments on publicly available datasets show that our model significantly outperforms state-of-the-art methods on image captioning and scene graph generation.


==> abstract.tex <==
% It is critical for humans to understand both the visual and the language world.
% Visual and Language Understanding are two promising research fields in artificial intelligence involving many challenging tasks, i.e., classification, detection, segmentation, natural language processing and generation, etc. 
% To truly understand the visual and language world our models should be able not only to recognize images and languages but also generate them.
% We focus on the generation tasks in three translation problems: image-to-image translation, language-to-language translation, and image-to-language translation.
% Translation problems usually involves two domains, source and target, which can be efficiently solved by using encoder-decoder structure with encoder encodes the source information and the decoder uses the source information to generate target image or language.
% This structure requires the encoding latent space to be well modeled because if not the generate target might be flawed or wrong.
% Thus, in this thesis, we target at exploring this latent space for generation tasks.
% We propose novel solutions to better explore the latent space by addressing the following problems.

% \begin{enumerate}
%     \item We solved the unsupervised multi-domain image-to-image translation problem using one Generative Adversarial Network (GAN). 
%     We used one encoder to encode information of all domains to the common latent space, starting from where, we generate to different domains with the guidance of domain labels.
%     \item We solved the neural machine translation (NMT) problem using Transformer. 
%     We explore the latent space of syntax and apply syntax in translation.
%     The translated sentence can be controlled by the generation of syntax.
%     \item We introduced a new problem of Fashion Captioning.
%     Given a fashion image, the model has to generate a detailed sentence to describe it.
%     We proposed to use semantics in language to help the generation of sentence.
%     The generated sentence has to contain as much semantic information as possible.
% \end{enumerate}


The interest in Artificial Intelligence (AI) and its applications has seen unprecedented growth in the last few years.
The success can be partly attributed to the advancements of deep neural networks made in the sub-fields of AI such as Computer Vision (CV) and Natural Language Processing (NLP). 
% The largest of the growths in these fields has been made possible with deep learning which uses the principles of deep neural networks. 
The promising research area that this dissertation focuses on is visual and language understanding which involves many challenging tasks, \textit{i.e.}, classification, detection, segmentation, machine translation and captioning, etc.
% As Richard Feynman said ``What I cannot create, I do not understand'', for a model to understand the visual and language world, it has to be capable to create new things based on what it has.
% The dissertation mainly focuses on using sequence to sequence (\texttt{Seq2Seq}) models to generate a target sentence to translate or describe a source sentence or image.
The state-of-the-art methods for solving these problems usually involves only two parts: source data and target labels, which is rather insufficient especially when the dataset is small.
Meanwhile, many external tools or sources can provide extra useful information (external knowledge) that can help improve the performance of these methods.
For example, a detection model has been applied to provide better object features than state-of-the-art ResNet for image captioning models.
Inspired by this observation, we developed a methodology that we can first extract external knowledge and then integrate it with the original models.
The external knowledge has to be extracted from the dataset, or can directly come from external, e.g., grammar rules or scene graphs.
We apply this methodology to different AI tasks, including machine translation and image captioning and improve the original state-of-the-art models by a large margin.
% In this work, we focus on using external tools to extract information from training data and integrate the extracted information with the original training models.


% The problems this work mainly targets on include but not limited to machine translation where a sentence of the target language is translated from a sentence of the source language and image captioning where a sentence is generated to describe a source image.
% These two problems can be directly solved by using sequence to sequence (\texttt{Seq2Seq}) models of the encoder-decoder architecture.
% Both encoder and decoder are modeled by using deep neural networks like convolutional neural network (CNN), recurrent neural network (RNN) or Transformer.
% However, in the real world scenarios, a lot of problems are associated with external knowledge.
% For example, sentences have the underlying Part-Of-Speech (POS) tags which are grammatical tags of words as nouns, verbs, adjectives, adverbs, etc.
% For images, however, the scene graphs are the hidden representation of the relations between the objects in the images.
% The specialty of different vision and language problems and the diversity of external knowledge representations determine that one single method for all problems is non-trivial.
% In this work, the author thus tries to propose various methods of exploring external knowledge to solve different language and vision problems to improve the effectiveness of the \texttt{Seq2Seq} methods.
% Evaluations on extensive experiments demonstrate the effectiveness of the different methods. 



==> acknowledgement.tex <==
I would like to acknowledge a number of people that have supported, in various ways, the creation of this work.

First and foremost, I’d like to express gratitude towards my advisor Prof. Xin Wang for accepting me as one of her PhD students in the year 2015. 
Xin gave me the opportunity to work on my research in relative peace, and our frequent discussions and brainstorming sessions were of key importance.
I could not have hoped for an advisor with a greater overlap in academic interests, possessing a greater intelligence or a greater clarity of thought. 
I also greatly admire that Xin manages to combine her qualities with a sense of responsibility. 
I would also like to thank Xin for providing the freedom to intern for a year performing research at different research labs in Silicon Valley, Seattle and New York City.

The colleague I interacted most with during my time at Stony Brook was Yingru Liu.
I would like to thank Yingru for weathering my frequent requests for feedbacks on various ideas.
I enjoyed our discussions while sitting in the lab, eating lunch at the cafeteria, self-studying in the library, and attending conferences at the Hilton Midtown.
It was always a pleasure to pick at his mind with new ideas, and his insights on generative deep learning were always thought-provoking.
In addition, I'd like to recognize Prof. Niranjan Balasubramanian for supervising me in finishing my neural machine translation paper, which was later accepted by EMNLP.

I was given the opportunity by research scientists Ran Xu and Jiangbo Yuan to spend two summers in 2017 and 2018 at the VIPShop AI Research Lab in Silicon Valley.
My time in California was formative, reinforcing my belief that this was the right field in which to pursue my doctoral degree.


I would also like to thank Jue Wang for hosting me at MEGVII Research during the summer of 2019.
It was a true pleasure brainstorming about sequence to sequence models and their role in the future of AI.
I also had the pleasure to collaborate with him and many others, resulting in our fashion captioning paper.

I'd like to thank Svebor Karaman and Joel Treault for having me at Dataminr during the summer of 2020.
Although we didn't have a chance to meet face to face because of the pandemic, their clear and deep insights into AI really impressed me and inspired me to be a better researcher.

I’d like to give credit to all the unnamed colleagues and friends who often endured my disorder and noise, and at other times provided me with much-needed moral support and distraction.

Finally and most importantly, I would like to acknowledge my parents and my brother for setting a great example and providing the best upbringing one could wish for.


\vspace{0.5in}

\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad Sincerely,
\vspace{0.5in}

\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad Xuewen Yang
\vspace{0.2in}

\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad Stony Brook

\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad USA

==> dedication.tex <==
\begin{spacing}{2.0}
To all my families and friends, \\
for their help and support in my life. 
\end{spacing}
